An Agnostic Approach to Building Empirical Type Ia Supernova Light Curves: Evidence for Intrinsic Chromatic Flux Variation Using Nearby Supernova Factory Data

We present a new empirical Type Ia supernova (SN Ia) model with three chromatic flux variation templates: one phase dependent and two phase independent. No underlying dust extinction model or patterns of intrinsic variability are assumed. Implemented with Stan and trained using spectrally binned Nearby Supernova Factory spectrophotometry, we examine this model's 2D, phase-independent flux variation space using two motivated basis representations. In both, the first phase-independent template captures variation that appears dust-like, while the second captures a combination of effectively intrinsic variability and second-order dust-like effects. We find that approximately 13% of the modeled phase-independent flux variance is not dust-like. Previous empirical SN Ia models either assume an effective dust extinction recipe in their architecture, or only allow for a single mode of phase-independent variation. The presented results demonstrate such an approach may be insufficient, because it could "leak" noticeable intrinsic variation into phase-independent templates.

==> sn_table2.tex <==
\begin{deluxetable*}{lrrrr}
\label{tab:sntab2}
\tablecaption{
    Selective extinction model derived per-SN parameter median values with 68\textsuperscript{th} percentile upper and lower values or standard deviation. 
    Note SNNGC2691 was dropped when calculated derived parameters to resolve covariance matrix rank deficiency (flagged N/A). 
    }
\tablehead{\colhead{SN} & \colhead{$c_a$} & \colhead{$c_b$} & \colhead{$\alpha_V$} & \colhead{$\rho_V$}}
\startdata
SN2011gf & -0.39$\pm$0.02 & -0.16$\pm$0.01 & -0.28$\pm$0.02 & 2.45$\pm$0.11 \\
SN2011ga & -0.11$\pm$0.02 & -0.04$\pm$0.01 & 0.01$\pm$0.01 & 20.45$\pm$37.09 \\
CSS130502\_01 & -0.31$\pm$0.02 & -0.13$\pm$0.01 & -0.19$\pm$0.03 & 2.23$\pm$0.15 \\
LSQ12fhe & -0.09$\pm$0.03 & -0.05$\pm$0.01 & 0.05$\pm$0.02 & 40.70$\pm$80.08 \\
LSQ14cnm & -0.22$\pm$0.02 & -0.09$\pm$0.01 & -0.11$\pm$0.02 & 2.35$\pm$0.24 \\
PTF09dlc & -0.15$\pm$0.02 & -0.05$\pm$0.01 & -0.01$\pm$0.02 & 13.54$\pm$23.94 \\
PTF09dnl & 0.06$\pm$0.02 & 0.03$\pm$0.01 & 0.18$\pm$0.02 & 2.57$\pm$0.17 \\
PTF09fox & -0.21$\pm$0.02 & -0.08$\pm$0.01 & -0.10$\pm$0.02 & 2.43$\pm$0.27 \\
PTF09foz & 0.12$\pm$0.02 & 0.05$\pm$0.01 & 0.24$\pm$0.02 & 2.64$\pm$0.16 \\
PTF10hmv & 0.26$\pm$0.02 & 0.11$\pm$0.01 & 0.38$\pm$0.02 & 2.58$\pm$0.11 \\
PTF10icb & 0.08$\pm$0.02 & 0.03$\pm$0.01 & 0.20$\pm$0.02 & 2.76$\pm$0.21 \\
PTF10mwb & 0.05$\pm$0.02 & 0.02$\pm$0.01 & 0.16$\pm$0.02 & 2.65$\pm$0.20 \\
PTF10nlg & 0.41$\pm$0.02 & 0.18$\pm$0.01 & 0.53$\pm$0.02 & 2.41$\pm$0.07 \\
PTF10qyz & -0.11$\pm$0.03 & -0.04$\pm$0.01 & 0.00$\pm$0.01 & 19.63$\pm$27.77 \\
PTF10wnm & -0.17$\pm$0.02 & -0.07$\pm$0.01 & -0.05$\pm$0.02 & 1.88$\pm$0.46 \\
PTF10wof & 0.02$\pm$0.03 & 0.02$\pm$0.01 & 0.14$\pm$0.03 & 2.38$\pm$0.19 \\
PTF11bgv & 0.08$\pm$0.02 & 0.03$\pm$0.01 & 0.20$\pm$0.03 & 3.06$\pm$0.30 \\
PTF11bju & -0.02$\pm$0.03 & -0.03$\pm$0.01 & 0.07$\pm$0.03 & 16.59$\pm$25.51 \\
PTF11bnx & 0.36$\pm$0.02 & 0.16$\pm$0.01 & 0.48$\pm$0.03 & 2.44$\pm$0.08 \\
PTF11mkx & -0.07$\pm$0.03 & -0.05$\pm$0.01 & 0.06$\pm$0.02 & 41.22$\pm$114.49 \\
PTF11mty & -0.21$\pm$0.02 & -0.09$\pm$0.01 & -0.09$\pm$0.02 & 2.16$\pm$0.29 \\
PTF12dxm & 0.23$\pm$0.02 & 0.09$\pm$0.01 & 0.35$\pm$0.03 & 2.63$\pm$0.13 \\
PTF12fuu & -0.32$\pm$0.02 & -0.13$\pm$0.01 & -0.21$\pm$0.02 & 2.35$\pm$0.13 \\
PTF12grk & 0.19$\pm$0.02 & 0.09$\pm$0.01 & 0.30$\pm$0.03 & 2.40$\pm$0.10 \\
PTF12iiq & 0.29$\pm$0.03 & 0.13$\pm$0.01 & 0.41$\pm$0.04 & 2.41$\pm$0.08 \\
PTF13anh & 0.12$\pm$0.03 & 0.06$\pm$0.01 & 0.23$\pm$0.03 & 2.39$\pm$0.12 \\
SN2004ef & 0.32$\pm$0.02 & 0.14$\pm$0.01 & 0.44$\pm$0.02 & 2.50$\pm$0.09 \\
SN2005hc & -0.15$\pm$0.02 & -0.06$\pm$0.01 & 0.00$\pm$0.03 & 10.32$\pm$21.46 \\
SN2005hj & -0.14$\pm$0.02 & -0.06$\pm$0.01 & -0.02$\pm$0.04 & 1.57$\pm$14.18 \\
SN2006cj & -0.21$\pm$0.02 & -0.09$\pm$0.01 & -0.10$\pm$0.02 & 2.10$\pm$0.27 \\
SN2007bd & -0.15$\pm$0.03 & -0.06$\pm$0.01 & 0.01$\pm$0.02 & 19.85$\pm$30.89 \\
SN2010dt & -0.12$\pm$0.02 & -0.04$\pm$0.01 & -0.00$\pm$0.01 & 19.40$\pm$33.28 \\
SN2012fr & -0.16$\pm$0.02 & -0.06$\pm$0.00 & -0.04$\pm$0.02 & 2.71$\pm$0.79 \\
SN2012dn & 0.07$\pm$0.02 & 0.02$\pm$0.01 & 0.18$\pm$0.03 & 3.36$\pm$0.43 \\
SNF20060512-001 & -0.08$\pm$0.02 & -0.04$\pm$0.01 & 0.04$\pm$0.02 & 29.40$\pm$46.65 \\
SNF20060526-003 & -0.08$\pm$0.02 & -0.03$\pm$0.01 & 0.01$\pm$0.02 & 14.04$\pm$40.90 \\
SNF20061020-000 & 0.12$\pm$0.03 & 0.04$\pm$0.01 & 0.23$\pm$0.03 & 2.84$\pm$0.23 \\
SNF20061021-003 & 0.09$\pm$0.02 & 0.04$\pm$0.01 & 0.21$\pm$0.02 & 2.58$\pm$0.16 \\
SNF20061022-005 & -0.08$\pm$0.03 & -0.04$\pm$0.01 & 0.04$\pm$0.02 & 27.55$\pm$33.31 \\
SNF20061111-002 & -0.08$\pm$0.03 & -0.03$\pm$0.01 & 0.01$\pm$0.02 & 22.45$\pm$190.03 \\
SNF20070424-003 & -0.07$\pm$0.02 & -0.02$\pm$0.01 & 0.01$\pm$0.02 & 9.83$\pm$21.98 \\
SNF20070506-006 & -0.23$\pm$0.02 & -0.10$\pm$0.01 & -0.12$\pm$0.03 & 2.05$\pm$0.25 \\
SNF20070630-006 & -0.04$\pm$0.02 & -0.01$\pm$0.01 & 0.06$\pm$0.03 & 2.63$\pm$0.54 \\
SNF20070717-003 & 0.22$\pm$0.02 & 0.10$\pm$0.01 & 0.34$\pm$0.02 & 2.45$\pm$0.10 \\
SNF20070802-000 & 0.25$\pm$0.02 & 0.11$\pm$0.01 & 0.37$\pm$0.03 & 2.43$\pm$0.09 \\
SNF20070818-001 & 0.19$\pm$0.02 & 0.09$\pm$0.01 & 0.31$\pm$0.03 & 2.40$\pm$0.10 \\
SNF20070831-015 & -0.06$\pm$0.03 & -0.02$\pm$0.01 & 0.02$\pm$0.02 & 19.24$\pm$31.88 \\
SNF20070902-018 & 0.17$\pm$0.03 & 0.07$\pm$0.01 & 0.29$\pm$0.03 & 2.70$\pm$0.16 \\
SNF20080507-000 & 0.11$\pm$0.02 & 0.04$\pm$0.01 & 0.23$\pm$0.03 & 2.73$\pm$0.19 \\
SNF20080510-001 & -0.14$\pm$0.02 & -0.06$\pm$0.01 & 0.00$\pm$0.02 & 17.09$\pm$30.15 \\
SNF20080510-005 & -0.19$\pm$0.03 & -0.08$\pm$0.01 & -0.04$\pm$0.05 & 2.23$\pm$11.45 \\
SNF20080512-010 & -0.05$\pm$0.02 & -0.03$\pm$0.01 & 0.04$\pm$0.02 & 18.70$\pm$27.80 \\
SNF20080514-002 & -0.18$\pm$0.02 & -0.08$\pm$0.01 & -0.06$\pm$0.02 & 1.62$\pm$0.42 \\
SNF20080522-000 & -0.21$\pm$0.02 & -0.10$\pm$0.01 & -0.09$\pm$0.03 & 1.69$\pm$0.33 \\
SNF20080522-011 & -0.26$\pm$0.02 & -0.10$\pm$0.01 & -0.15$\pm$0.02 & 2.44$\pm$0.18 \\
SNF20080531-000 & 0.00$\pm$0.02 & 0.01$\pm$0.01 & 0.12$\pm$0.02 & 2.49$\pm$0.24 \\
SNF20080614-010 & 0.14$\pm$0.02 & 0.05$\pm$0.01 & 0.26$\pm$0.03 & 2.79$\pm$0.20 \\
SNF20080620-000 & 0.16$\pm$0.02 & 0.07$\pm$0.01 & 0.28$\pm$0.03 & 2.57$\pm$0.13 \\
SNF20080626-002 & -0.12$\pm$0.02 & -0.05$\pm$0.01 & -0.00$\pm$0.01 & 30.15$\pm$51.00 \\
SNF20080714-008 & 0.41$\pm$0.02 & 0.18$\pm$0.01 & 0.54$\pm$0.02 & 2.42$\pm$0.07 \\
SNF20080725-004 & 0.01$\pm$0.02 & 0.01$\pm$0.01 & 0.12$\pm$0.03 & 2.42$\pm$0.22 \\
SNF20080803-000 & 0.22$\pm$0.02 & 0.09$\pm$0.01 & 0.34$\pm$0.03 & 2.55$\pm$0.11 \\
SNF20080810-001 & 0.03$\pm$0.02 & 0.01$\pm$0.01 & 0.15$\pm$0.02 & 3.19$\pm$0.38 \\
SNF20080821-000 & -0.06$\pm$0.02 & -0.02$\pm$0.01 & 0.03$\pm$0.03 & 7.97$\pm$17.29 \\
SNF20080825-010 & -0.05$\pm$0.02 & -0.02$\pm$0.01 & 0.05$\pm$0.03 & 6.94$\pm$12.17 \\
SNF20080909-030 & -0.07$\pm$0.04 & -0.03$\pm$0.02 & 0.03$\pm$0.02 & 22.55$\pm$39.37 \\
SNF20080913-031 & 0.13$\pm$0.06 & 0.06$\pm$0.03 & 0.23$\pm$0.06 & 2.54$\pm$0.21 \\
SNF20080918-000 & 0.27$\pm$0.03 & 0.12$\pm$0.01 & 0.39$\pm$0.03 & 2.50$\pm$0.10 \\
SN2011hr & N/A & N/A & N/A & N/A \\
SN2011bc & 0.29$\pm$0.02 & 0.12$\pm$0.01 & 0.42$\pm$0.03 & 2.53$\pm$0.10 \\
SN2012cg & 0.17$\pm$0.02 & 0.07$\pm$0.01 & 0.29$\pm$0.03 & 2.71$\pm$0.16 \\
SN2013bt & -0.07$\pm$0.02 & -0.04$\pm$0.01 & 0.04$\pm$0.02 & 52.46$\pm$172.21 \\
SN2011be & -0.30$\pm$0.03 & -0.13$\pm$0.01 & -0.18$\pm$0.03 & 2.21$\pm$0.16
\enddata
\end{deluxetable*}


==> sn_table2_10entries.tex <==
\begin{deluxetable*}{lrrrr}
\label{tab:sntab2}
\tablecaption{
    Selective extinction model derived per-SN parameter median values with 68\textsuperscript{th} percentile upper and lower values or standard deviation for our first 10 SNe~Ia. 
    Note SNNGC2691 was dropped when calculated derived parameters to resolve covariance matrix rank deficiency (flagged N/A). 
    A corresponding full table of all training SNe~Ia is available upon request. 
    }
\tablehead{\colhead{SN} & \colhead{$c_a$} & \colhead{$c_b$} & \colhead{$\alpha_V$} & \colhead{$\rho_V$}}
\startdata
SN2011gf & -0.39$\pm$0.02 & -0.16$\pm$0.01 & -0.28$\pm$0.02 & 2.45$\pm$0.11 \\
SN2011ga & -0.11$\pm$0.02 & -0.04$\pm$0.01 & 0.01$\pm$0.01 & 20.45$\pm$37.09 \\
CSS130502\_01 & -0.31$\pm$0.02 & -0.13$\pm$0.01 & -0.19$\pm$0.03 & 2.23$\pm$0.15 \\
LSQ12fhe & -0.09$\pm$0.03 & -0.05$\pm$0.01 & 0.05$\pm$0.02 & 40.70$\pm$80.08 \\
LSQ14cnm & -0.22$\pm$0.02 & -0.09$\pm$0.01 & -0.11$\pm$0.02 & 2.35$\pm$0.24 \\
PTF09dlc & -0.15$\pm$0.02 & -0.05$\pm$0.01 & -0.01$\pm$0.02 & 13.54$\pm$23.94 \\
PTF09dnl & 0.06$\pm$0.02 & 0.03$\pm$0.01 & 0.18$\pm$0.02 & 2.57$\pm$0.17 \\
PTF09fox & -0.21$\pm$0.02 & -0.08$\pm$0.01 & -0.10$\pm$0.02 & 2.43$\pm$0.27 \\
PTF09foz & 0.12$\pm$0.02 & 0.05$\pm$0.01 & 0.24$\pm$0.02 & 2.64$\pm$0.16 \\
PTF10hmv & 0.26$\pm$0.02 & 0.11$\pm$0.01 & 0.38$\pm$0.02 & 2.58$\pm$0.11
\enddata
\end{deluxetable*}


==> sn_table_10entries.tex <==
\begin{deluxetable*}{lrrrrrrr}
\tablecaption{
    Model per-SN parameter median values with 68\textsuperscript{th} percentile upper and lower valuesn for our first 10 SNe~Ia. 
    Per-SN parameters $$\chi_0 - \langle \chi_0 \rangle$$, $s_1$, $c_1$, and $c_2$ have been transformed to magnitudes. 
    A full table of all training SNe~Ia is available upon request. 
    }
\tablehead{\colhead{SN} & \colhead{$\chi_0 - \langle \chi_0 \rangle$} & \colhead{$s_1$} & \colhead{$c_1$} & \colhead{$c_2$} & \colhead{$t_0$}}
\startdata
\label{table:table1}
SNF20060512-001 & $-0.04\pm0.03$ & $-0.02\pm0.01$ & $-0.33\pm0.09$ & $0.12\pm0.03$ & $53882.5\pm0.12$ \\
SNF20060526-003 & $-0.06\pm0.03$ & $-0.07\pm0.01$ & $-0.31\pm0.09$ & $-0.04\pm0.02$ & $53893.4\pm0.21$ \\
SNF20061020-000 & $0.30\pm0.03$ & $0.21\pm0.01$ & $0.44\pm0.11$ & $0.08\pm0.03$ & $54037.9\pm0.19$ \\
SNF20061021-003 & $-0.08\pm0.03$ & $-0.05\pm0.01$ & $0.38\pm0.08$ & $-0.04\pm0.02$ & $54039.7\pm0.13$ \\
SNF20061022-005 & $-0.11\pm0.03$ & $-0.08\pm0.02$ & $-0.34\pm0.10$ & $0.15\pm0.03$ & $54040.8\pm0.17$ \\
SNF20061111-002 & $0.08\pm0.03$ & $-0.01\pm0.01$ & $-0.30\pm0.12$ & $-0.05\pm0.03$ & $54060.8\pm0.18$ \\
SNF20070424-003 & $0.08\pm0.03$ & $-0.05\pm0.01$ & $-0.26\pm0.09$ & $-0.07\pm0.02$ & $54225.8\pm0.16$ \\
SNF20070506-006 & $-0.19\pm0.03$ & $-0.07\pm0.01$ & $-0.94\pm0.08$ & $0.09\pm0.02$ & $54245.9\pm0.10$ \\
SNF20070630-006 & $-0.09\pm0.02$ & $-0.04\pm0.01$ & $-0.16\pm0.08$ & $-0.06\pm0.02$ & $54294.9\pm0.11$ \\
SNF20070717-003 & $-0.12\pm0.02$ & $0.03\pm0.01$ & $0.90\pm0.08$ & $-0.12\pm0.02$ & $54310.3\pm0.11$
\enddata
\end{deluxetable*}

